Scalability Analysis of Direct and Iterative Solvers Used to Model Charging of Non-insulated Superconducting Pancake Solenoids

A mathematical model for the charging simulation of non-insulated superconducting pancake solenoids is presented. Numerical solutions are obtained by the simulation model implemented on the Petra-M FEM platform using a variety of solvers. A scalability analysis is performed for both direct and preconditioned iterative solvers for four different pancakes solenoids with a varying number of turns and mesh elements. It is found that even with two extremely different time scales in the system an iterative solver combination (FGMRES-GMRES) in conjunction with the parallel Auxiliary Space Maxwell Solver (AMS) preconditioner outperforms a parallelized direct solver (MUMPS). In general, the computational time of the iterative solver is found to increase with the number of turns in the solenoids and/or the conductivity assumed for the superconducting material.

==> notation.tex <==
\newcommand{\EX}{{\Bbb{E}}}
\newcommand{\PX}{{\Bbb{P}}}

% \left \right 
\newcommand{\lp}{\left(}
\newcommand{\rp}{\right)}
\newcommand{\lb}{\left[}
\newcommand{\rb}{\right]}
\newcommand{\lbr}{\left\{}
\newcommand{\rbr}{\right\}}
\newcommand{\lnorm}{\left\|}
\newcommand{\rnorm}{\right\|}

% environments
\newtheorem{remark}{Remark}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{assumption}{Assumption}[section]



\def\PP{{{\rm l}\kern - .15em {\rm P} }}
\def\PN2{{\PP_{N}-\PP_{N-2}}}

\newcommand{\erf}[1]{\mbox{erf}\left(#1\right)}

% math symbols
\newcommand{\D}{\mathbbm{D}}
\newcommand{\I}{\mathbbm{I}}
\newcommand{\N}{\mathbbm{N}}
\newcommand{\R}{\mathbbm{R}}
\newcommand{\Z}{\mathbbm{Z}}

% calligraphic letters
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}


% boldface Greek letters
\newcommand{\bfeta}{\boldsymbol{\eta}}
\newcommand{\bLambdar}{\boldsymbol{\Lambda}_r}
\newcommand{\bLambdarL}{\boldsymbol{\Lambda}_r^{L^2}}
\newcommand{\bLambdarH}{\boldsymbol{\Lambda}_r^{H^1}}
\newcommand{\bPhi}{\boldsymbol{\Phi}}
\newcommand{\bPhir}{\boldsymbol{\Phi}_r}
\newcommand{\bphi}{\boldsymbol{\varphi}}
\newcommand{\bphir}{\boldsymbol{\varphi}_r}
\newcommand{\bPsi}{\boldsymbol{\Psi}}
\newcommand{\btau}{\boldsymbol{\tau}}

% boldface letters
\newcommand{\ba}{\boldsymbol{a}}
\newcommand{\bas}{{\boldsymbol a}^{snap}}
\newcommand{\bA}{\boldsymbol{A}}
\newcommand{\bb}{\boldsymbol{b}}
\newcommand{\bB}{\boldsymbol{B}}
\newcommand{\bc}{\boldsymbol{c}}
\newcommand{\bd}{\boldsymbol{d}}
\newcommand{\be}{\boldsymbol{e}}
\newcommand{\bff}{\boldsymbol{f}}
\newcommand{\bFF}{{\boldsymbol F}}
\newcommand{\bG}{{\boldsymbol G}}
\newcommand{\bGs}{{\boldsymbol G}^{snap}}
\newcommand{\bh}{\boldsymbol{h}}
\newcommand{\bH}{\boldsymbol{H}}
\newcommand{\bL}{\boldsymbol{L}}
\newcommand{\bM}{\boldsymbol{M}}
\newcommand{\bq}{{\boldsymbol q}}
\newcommand{\bqs}{{\boldsymbol q}^{snap}}
\newcommand{\br}{\boldsymbol{r}}
\newcommand{\bS}{\boldsymbol{S}}
\newcommand{\bu}{\boldsymbol{u}}
\newcommand{\bU}{\boldsymbol{U}}
\newcommand{\bur}{{\boldsymbol{u}}_r}
\newcommand{\bUr}{{\boldsymbol{U}}_r}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\bV}{\boldsymbol{V}}
\newcommand{\bvr}{{\boldsymbol{v}}_r}
\newcommand{\bw}{\boldsymbol{w}}
\newcommand{\bW}{\boldsymbol{W}}
\newcommand{\bwr}{{\boldsymbol{w}}_r}
\newcommand{\bWr}{{\boldsymbol{W}}_r}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\bX}{\boldsymbol{X}}
\newcommand{\bXh}{{\bf X}^h}
\newcommand{\bXr}{{\bf X}^r}
\newcommand{\bY}{\boldsymbol{Y}}
\newcommand{\bz}{\boldsymbol{z}}

% tilde letters
\newcommand{\tA}{\tilde{A}}
\newcommand{\tB}{\widetilde{B}}


% overline letters
\newcommand{\oa}{\overline{a}}
\newcommand{\oA}{\overline{A}}
\newcommand{\oc}{\overline{c}}
\newcommand{\obc}{\overline{\boldsymbol c}}
\newcommand{\op}{\overline{p}}
\newcommand{\oU}{\overline{U}}
\newcommand{\obu}{\overline{\boldsymbol u}}
\newcommand{\obU}{\overline{\boldsymbol U}}
\newcommand{\obur}{\overline{\boldsymbol{u}_r}}
\newcommand{\obUr}{\overline{\boldsymbol{U}_r}}
\newcommand{\obv}{\overline{\boldsymbol v}}
\newcommand{\obx}{\overline{\boldsymbol x}}
\newcommand{\ob}[1]{\overline{\boldsymbol{#1}}}
\newcommand{\orr}[1]{\overline{#1}^r}
\newcommand{\obr}[1]{\overline{\boldsymbol{#1}}^r}
\newcommand{\oh}[1]{\overline{#1}^h}
\newcommand{\obh}[1]{\overline{\boldsymbol{#1}}^h}

% POD notation
\newcommand{\as}{a^{snap}}
\newcommand{\CinvNabla}{C_{inv}^{\nabla}(r)}
\newcommand{\CinvDelta}{C_{inv}^{\Delta}(r)}
\newcommand{\Deltar}{\Delta_r}
\newcommand{\Gs}{G^{snap}}
\newcommand{\ct}{\bu_h^{avg}}



\newcommand{\bus}{{\bf u}^*}
\newcommand{\By}{\mathcal B(\by)}
\newcommand{\eci}[1]{\mathcal E_{#1}}
\newcommand{\dpyi}[1]{\delta_{#1}^+(\by)}
\newcommand{\dmyi}[1]{\delta_{#1}^-(\by)}
\newcommand{\cA}{{\mathcal A(\by)}}
\newcommand{\dyi}[1]{\delta_{#1}(\by)}
\newcommand{\cG}{{\mathcal G(\bx,\by)}}
\newcommand{\cGi}[1]{{\mathcal G_{#1}(\bx,\by)}}
\newcommand{\pti}{\partial_i}
\newcommand{\ptii}[1]{\partial_{#1}}
\newcommand{\vertiii}[1]{{|\!|\!| #1 |\!|\!|}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% colors
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\blue}[1]{{\color{blue}#1}}
\newcommand{\inserted}[1]{\blue{#1}}
\newcommand{\deleted}[1]{{}}%\color{red}{#1}}}
%\newcommand{\comment}[1]{{\color{cyan}#1}}

% fractions
\newcommand{\half}{\frac{1}{2}}



